Scaling up statistical model checking of cyber-physical systems via algorithm ensemble and parallel simulations over HPC infrastructures

Model-based formal verification of industry-relevant Cyber-Physical Systems (CPSs) is often a computationally prohibitive task. In most cases, the complexity of the models precludes any prospect of symbolic analysis, leaving numerical simulation as the only viable option. Unfortunately, exhaustive simulation of a CPS model over the entire set of plausible operational scenarios is rarely possible in practice, and alternative strategies such as Statistical Model Checking (SMC) must be used instead. In this article, we show that the number of model simulations (samples) required by SMC techniques to converge can be significantly reduced by considering multiple (an ensemble of) Adaptive Stopping Algorithms (SAs) at once, and that the simulations themselves (by far the most expensive step of the entire workload) can be efficiently sped up by exploiting massively parallel platforms. With three industry-scale CPS models, we experimentally show that the use of an ensemble of two state-of-the-art SAs (AA and EBGStop) may require dozens of millions fewer samples when compared to running a single algorithm, with reductions in sample size of up to 78%. Furthermore, we show that our implementation, by massively parallelizing system model simulations on a HPC infrastructure, yields speed-ups for the completion time of the verification tasks which are practically linear with respect to the number of computational nodes, thus achieving an efficiency of virtually 100%, even on very large platforms. This makes it possible to complete tasks of model-based SMC verification for complex CPSs in a matter of hours or days, whereas a na\"ive sequential execution would require from months to many years.

==> 00-preamble-acronyms.tex <==
%!TEX root = ../root.tex


% Low-level syntax allowed by MCLabPaper_Minimal.sty (wrt. MCLabPaper.sty)
%\NewAcronym{id}{short}{short plural}{long}{long plural}

\NewAcronym{ALMA}
	{ALMA}
	{ALMA}
	{Apollo Lunar Module Autopilot}
	{Apollo Lunar Module Autopilot}
\NewAcronym{HPC-EAA}
	{HPC-EAA}
	{HPC-EAA}
	{EAA with Parallel Scenario Evaluation over HPC}
	{EAA with Parallel Scenario Evaluation over HPC}
\NewAcronym{AT}
	{AT}
	{AT}
	{Automatic Transmission}
	{Automatic Transmission}
\NewAcronym{CPS}
	{CPS}
	{CPSs}
	{Cyber-Physical System}
	{Cyber-Physical Systems}
\NewAcronym{EAA}
	{EAA}%{\protect{\ensuremath{\mathcal{EAA}}}}
	{EAA}%{\protect{\ensuremath{\mathcal{EAA}}}}
	{Ensemble of Approximation Algorithms}
	{Ensemble of Approximation Algorithms}
\NewAcronym{FCS}
	{FCS}
	{FCS}
	{Fuel Control System}
	{Fuel Control Systems}
\NewAcronym{HPC}
	{HPC}
	{HPC}
	{High-Performance Computing}
	{High-Performance Computing}
\NewAcronym{iid}
	{iid}
	{iid}
	{independent and identically distributed}
	{independent and identically distributed}
\NewAcronym{KPI}
	{KPI}
	{KPIs}
	{Key Performance Indicator}
	{Key Performance Indicators}
\NewAcronym{MTBF}
	{MTBF}
	{MTBF}
	{Mean Time Between Failures}
	{Mean Time Between Failures}
\NewAcronym{MPI}
	{MPI}
	{MPI}
	{Message Passing Interface}
	{Message Passing Interface}	
\NewAcronym{SA}
	{SA}
	{SAs}
	{Adaptive Stopping Algorithm}
	{Adaptive Stopping Algorithms}
\NewAcronym{sampler}
	{APSG}
	{APSGs}
	{Asynchronous Parallel Sample Generator}
	{Asynchronous Parallel Sample Generators}	
\NewAcronym{SMC}
	{SMC}
	{SMC}
	{Statistical Model Checking}
	{Statistical Model Checking}
\NewAcronym{SUV}
	{SUV}
	{SUVs}
	{System Under Verification}
	{Systems Under Verification}


==> 00-preamble-database.tex <==
%!TEX root = ../root.tex

% AT
\DataPut{case studies/at/sim time/avg} % avg sim time
	{\Pretty[s]{0.1377}}%0.13769579797896003}}
\DataPut{case studies/at/sim time/stddev} % stddev of sim time
	{\Pretty[s]{0.03696}}%0.03695578288780998
\DataPut{case studies/at/scenarios/max}	% max_{eps,delta} EAA.nb_scenarios
	{\Pretty{11047532}}
% \DataPut{case studies/at/ensamble/scenarios/saving/max} % max_{e,d} saving%
% 	{\Pretty[\%]{99.99}}




% FCS
\DataPut{case studies/fcs/sim time/avg}
	{\Pretty[s]{0.2279}} %0.22791278083878524
\DataPut{case studies/fcs/sim time/stddev}
	{\Pretty[s]{0.0370}}%0.03695578288780998
\DataPut{case studies/fcs/scenarios/max}
	{\Pretty{10091091}}
% \DataPut{case studies/fcs/ensamble/scenarios/saving/max}
% 	{\Pretty[\%]{99.99}}





% ALMA
\DataPut{case studies/alma/sim time/avg}
	{\Pretty[s]{7.1654}}%7.165403056105263
\DataPut{case studies/alma/sim time/stddev}
	{\Pretty[s]{2.6291}}%2.629132216833615
\DataPut{case studies/alma/scenarios/max}
	{\Pretty{102065528}}
% \DataPut{case studies/alma/ensamble/scenarios/saving/max}
% 	{\Pretty[\%]{99.99}}



\DataPut{exps/eaa/samples reduction/max}{\Pretty{31300400}}
\DataPut{exps/eaa/samples reduction/max/perc}{\ensuremath{78.73\%}}


% avg network turnaround time per sample
% \DataPut{exps/time/network/avg}
% 	{\Pretty[s]{0.9999}}
\DataPut{exps/time/network/scenarios/nb}% nb of scenarios used for the statistics.
	{1 million}


\DataPut{sw/repo}{\noexpand\url{https://bitbucket.org/mclab/tool-scalingup-smc-jss-2024/src/main/}}

==> 00-preamble-notation.tex <==
%!TEX root = ../root.tex

% Algos
\newcommand{\Algo}{\ensuremath{\mathcal{A}}\xspace}
\newcommand{\ApproxAlgo}{\ensuremath{\mathcal{AA}}\xspace}
\newcommand{\EBStop}{EBStop\xspace}
\newcommand{\EBGStop}{EBGStop\xspace}
\newcommand{\EAA}{{\Acs{EAA}}\xspace}

% SMC
\newcommand{\Prob}{\ensuremath{\Fun{P}}}
\newcommand{\Estimator}[1]{\ensuremath{\hat{#1}}}
\newcommand{\CyclicalEstimator}[1]{\ensuremath{\mathring{#1}}}
\newcommand{\DynEstimator}[1]{\ensuremath{\check{#1}}}
\newcommand{\Expectation}{\ensuremath{\mathbb{E}}}
\newcommand{\Precision}{\ensuremath{\varepsilon}\xspace}
\newcommand{\ConfMargin}{\ensuremath{\delta}\xspace}
\newcommand{\Mean}{\ensuremath{\mu}}
\newcommand{\PrecConf}{\ensuremath{(\Precision,\ConfMargin)}}


% CPSs
\newcommand{\SUV}{\ensuremath{\mathcal{S}}}
\newcommand{\TimeSet}{\ensuremath{\mathcal{T}}}
\newcommand{\InSpace}{\ensuremath{U}}
\let\InputSpace\InSpace
\newcommand{\OutSpace}{\ensuremath{O}}
\let\OutputSpace\OutSpace
\newcommand{\SimFun}{\ensuremath{S}}
\newcommand{\InFun}{\ensuremath{\Fun{u}}}
\let\InputFunction\InFun
\newcommand{\OutFun}{\ensuremath{\Fun{o}}}
\newcommand{\SUVDef}{\ensuremath{(\TimeSet, \InputSpace, \OutputSpace, \SimFun)}}

% Simulation
\newcommand{\Horizon}{\ensuremath{h}}

% Environments
\newcommand{\EnvInputSet}{\ensuremath{\mathbb{U}}}
\newcommand{\EnvInputSetParamSpace}{\ensuremath{\Lambda}}
\newcommand{\EnvProb}{\ensuremath{\Prob}}
\newcommand{\Env}{\ensuremath{\Fun{Env}}}
\newcommand{\EnvDef}{\ensuremath{(\EnvInputSet, \EnvProb)}}



% KPI
\newcommand{\KPI}{\ensuremath{\kappa}}
\newcommand{\Threshold}{\ensuremath{\vartheta}}


% Implementation
\newcommand{\AlgoNb}{\ensuremath{k}}
\newcommand{\SimNb}{\ensuremath{n}}


% Experiments
\newcommand{\Rate}[1]{\ensuremath{\rho_{#1}}}
\newcommand{\RateEAA}{\ensuremath{\rho_{_\text{\Acs{EAA}}}}}
\newcommand{\RateSampler}[1]{\ensuremath{\rho_{_\text{\Acs{sampler}, #1}}}}


==> 00-preamble-style.tex <==
%!TEX root = ../root.tex
\RestyleAlgo{ruled}
\SetInd{0.5em}{0.5em}

\renewcommand{\AlgoFun}[1]{\textsl{#1}}
\renewcommand{\AlgoVar}[1]{\textsl{#1}}


==> 01-introduction-contribution.tex <==
%!TeX root = ../../root.tex
%
In this article, we address the limitations of model-based verification of \Acp{CPS} via \Ac{SMC} in two ways:

\begin{enumerate}
	\item We propose \Ac{EAA}, a composite algorithm that concurrently runs a set (\emph{ensemble}) of different \Acp{SA}, by feeding them all with the same sequence of \Ac{iid} samples, and terminating as soon as the first \Ac{SA} of the ensemble converges with an approximation of the quantity of interest satisfying the requested statistical guarantees.

	\item We show a very effective architecture that exploits \Ac{HPC} infrastructures to speed-up the generation of samples via the use of many identical simulators running in parallel, still guaranteeing that the generated sequence of samples is \emph{identical} to the sequence that would be generated by a sequential sampler (if launched with the same random seed). This avoids any bias in the (pseudo-)randomness of the samples and so in the final result of the approximation.
\end{enumerate}	

We present our implementation combining two of the most well-known \Acp{SA} as an ensemble, \EBGStop \cite{mnih2008empirical} and \ApproxAlgo \cite{dagum2000optimal}, and evaluate its performance by conducting simulation-based \Ac{SMC}-driven verification of Simulink/Stateflow models of three \Acp{CPS} of industrial size: 
\Ac{AT},
\Ac{FCS}
and 
\Ac{ALMA}.

We emphasize that \Ac{EAA} can be seamlessly applied to virtually any \Ac{SMC} task, beyond the verification of \Acp{CPS}. 
However, in this article, we explicitly focus on model-based \Ac{CPS} verification, since in this setting sample size minimization is crucial, given the high cost of generating each sample (which entails the numerical simulation of the system model).

In this context, we show that exploiting \Ac{EAA} can significantly reduce the number of necessary samples (requiring up to \DataGet{exps/eaa/samples reduction/max} and up to \DataGet{exps/eaa/samples reduction/max/perc} fewer samples) when compared to running a single \Ac{SA}, and that our implementation for parallel samples generation shows an efficiency very close to $100\%$, even when using large platforms.
Overall, the combined effect of using \Ac{EAA} and of massively parallelizing the samples generation process allows us to carry out in a matter of hours or days \Ac{SMC}-based verification tasks for our case studies that would have taken months or even many years to complete if run sequentially.



==> 01-introduction-motivation.tex <==
%!TEX root = ../../root.tex
%
Designing experiments and protocols which minimize the size of a required sample is a very old problem in statistics \cite{singh2014sampling}. Hence, many techniques have already been developed to improve the sampling strategies in the context of \Ac{SMC} in order to reduce the number of required samples (see \cite{barbot2012coupling,jegourel2012cross,d2015smart,parmentier2023optimized} for some examples).

One such techniques is the use of \emph{\Acp{SA}}, \ie approximation algorithms that do not fix the number of required samples in advance, but continuously monitor their own progress and gradually ask for new samples until enough knowledge has been accumulated to compute an approximation of the quantity of interest with the sought statistical properties. 
%
Some \Acp{SA} have been proven to be \emph{optimal}, in that they are probabilistically guaranteed to stop after a number of samples which is always within a constant factor from the minimum number of samples theoretically needed to compute the requested approximation.

\Acp{SA} can be applied in an extremely large range of situations since they only modify the sampling process. 
For example, they have been used to scale up machine learning algorithms \cite{bradley2007filterboost} or to offer an efficient solution to the multi-armed bandit problem \cite{audibert2007tuning,even2002pac}. They have been extensively studied for their applications for \Ac{SMC} as well \cite{domingo2000madaboost,domingo2002,mnih2008empirical,dagum2000optimal}.

Introducing parallelization to \Ac{SMC} algorithms can seem to be an obvious solution to enhance their performance and scale of use. 
While in some cases \cite{alturki2011pvesta,pappagallo2020pmonte}, this has been done with great results, the complexity of most of the more advanced techniques of \Ac{SMC} makes it often very difficult to implement at best, or fundamentally impossible at worst \cite{bulychev2011distributed}. However, it turns out that since \Acp{SA} only focus on and determine the sampling process itself, without even having any restriction as to how the samples are produced, \Acp{SA} are not just efficient at minimizing the sample size, but are also highly modular and well-suited to be parallelized.

The various \Acp{SA} available (some of them are described in \cref{sec:preliminaries:sa}) mainly differ with respect to the statistical result exploited to derive their stopping criterion. 
%
As a consequence, they may require a fewer or a higher number of samples to converge, depending on various aspects of the problem at hand. %, also depending on the statistical properties of the quantity of interest.

In the case of model-based \Ac{SMC}-driven verification of \Acp{CPS}, generating each sample is particularly expensive, as this typically requires to numerically simulate the system model under an operational scenario randomly chosen from some distribution, in order to compute the value of a specific \Ac{KPI}.
%
Thus, overshooting the size of the sample by a large margin can have a critical impact on the running time of the approximation algorithm. 
If the system deals with online processes, this can even completely invalidate the verification task. 

To compute approximations of a system \Ac{KPI} as fast and as efficiently as possible, one needs to select the \Ac{SA} which would stop after the smallest possible number of samples for the problem at hand.
%
Unfortunately, the number of samples needed by any given \Ac{SA} to converge depends not only on the requested properties of the approximation, but also on statistical properties of the \Ac{KPI} of interest, which are typically unknown \emph{a priori}.


==> 01-introduction-outline.tex <==
%!TEX root = ../../root.tex
This article is organized as follows. 
\Cref{sec:background} presents preliminaries and discusses state-of-the-art \Acp{SA}, with a special emphasis on \EBStop and \ApproxAlgo. 
\Cref{sec:formal-framework} defines the formal framework used throughout the article.
\Cref{sec:eaa} and \cref{sec:hpc-eaa} describe \Ac{EAA} and our massively parallel implementation, respectively.
\Cref{sec:expres} is devoted to the experimental analysis of our algorithm and parallel tool. 
Finally, \cref{sec:conclusions} draws conclusions and perspectives.


==> 01-introduction.tex <==
%!TEX root = ../root.tex
%
The growing need for tools designed for the formal verification of complex systems faces a fundamental problem of scalability. 
In particular, for \Acp{CPS} \cite{clarke2011statistical}, \ie systems with physical components which are monitored and controlled by integrated computer entities to execute a specific task safely and effectively (most often in a dynamic fashion and in a nondeterministic environment), exhaustive methods of model checking are basically always impossible to apply. For instance, even the simplest model of a prototype for a self-driving vehicle will have too many states and possible paths of executions for any comprehensive algorithm to be run within a realistic time frame. This is due to the state-explosion problem \cite{clarke2012model}: the size of a state-based model scales exponentially with the number of variables used to represent the system.

Therefore, stochastic algorithms must be used instead. 
\Ac{SMC} \cite{larsen2016statistical} offers a wide range of frameworks and probabilistic methods to analyze and verify large models of complex systems. 
%
While these tools generally cannot provide definite answers to verification problems, they can actually be applied to real-world use-cases and generate approximations of \Acp{KPI} of the system which come with user-defined probabilistic guarantees.
%
\Ac{SMC}, sometimes in conjunction with machine learning \cite{larsen2022formal}, has for instance been successfully exploited for the validation and verification or privacy- and security-sensitive structures, such as railway signalling systems or information sharing platforms for healthcare \cite{basile2022exploring,baranov2021secure}. 

\SectionInput
	{Motivation}
	{01-introduction-motivation.tex}

\SectionInput
	[sec:intro:contribution]
	{Contribution}
	{01-introduction-contribution.tex}

\SectionInput
	{Outline}
	{01-introduction-outline.tex}



==> 02-background-estimators.tex <==
%!TEX root = ../root.tex
Given a real-valued random variable $X$, an estimator $\Estimator{p}$ for one of its parameters $p$ is \emph{unbiased} if $\Expectation(\hat{p}) = p$. 
The estimator is an \PrecConf-estimator if for any precision $\Precision \in (0,1)$ and confidence margin $\ConfMargin \in (0,1)$, there exists a sample size $N_{(\Precision, \ConfMargin)}$ such that the produced estimation is within $[p(1-\Precision), p(1+\Precision)]$ with a probability greater than $1-\ConfMargin$. Such an approximation is called a \PrecConf-approximation.

In the case of the expected value of a random variable $X$, the classic sample mean estimator is the go-to estimator. 
If sampling is performed with respect to the distribution of $X$, it is an unbiased estimator. 
In that case, it follows directly from the central limit theorem that it is an \PrecConf-estimator as well. 

==> 02-background-stopping-algorithms.tex <==
%!TEX root = ../root.tex
Classical estimation algorithms for the expected value of a random variable, such as Monte-Carlo algorithms, fully determine their sample size \emph{a priori}, for instance by exploiting the Chernoff bound \cite{clarke2011statistical,boyer2013plasma,agha2018survey}. 
This approach suffers from three key weaknesses: 
(a)~it is completely agnostic with respect to the random variable under study, 
(b)~it can overshoot the size of the required sample by a large margin, and 
(c)~it is not updated and improved during the execution of the algorithm. 

\emph{\Acp{SA}} are approximation algorithms that have none of those issues. 
They are designed so to require an as small as possible sample size for the computation of the sought approximation. 
They manage to do so by not only exploiting more advanced results of statistics, such as the Hoeffding's inequality \cite{domingo2000madaboost}, and ideas inspired from the theory of sequential testing, but also by continuously updating their stopping criterion with the information that they have already accumulated at any step to decide whether they have reached a sample size which will guarantee a \PrecConf-approximation.

\Cref{algo:sa} is an example of a generic and simplified \Ac{SA} which outputs an \PrecConf-approximation of the expected value of random variable $X$. The defining characteristic of an \Ac{SA} is its \emph{stopping criterion}: the algorithm loops and progressively acquires a larger and larger sample, updating the estimation $\Estimator{\Mean}$ and the stopping criterion itself at each step, until the test of the stopping criterion is finally satisfied, at which point the sample size ensures that $\Estimator{\Mean}$ is an \PrecConf-approximation of $\Expectation(X)$.


   \begin{algorithm}
      \caption{Generic \Acf{SA}}
      \label{algo:sa}
      \KwIn: random variable $X$\; 
      \KwIn: $\Precision, \ConfMargin \in (0,1)$\;
      \AlgoVarGets{$t$}{0}\;
      \AlgoVarGets{samples}{$\emptyset$}\;
      \Repeat{stopping criterion satisfied}{
         \AlgoVarIncr{$t$}\;
         \AlgoVarGets{samples}{$\AlgoVar{samples} \cup \Set{x_t}$}\;
         \AlgoVarGets{$\Estimator{\Mean}$}{mean(samples)}\;
         update stopping criterion\;
      }
      \Return{$\Estimator{\Mean}$}\;
   \end{algorithm} 


The fact that the stopping criterion of a \Ac{SA} depends on and takes into account (the realizations $x_t$ of) the random variable and that it is constantly updated throughout the progress of the algorithm is necessary but is not enough in itself to guarantee that the final sample size will not be larger than necessary. 
This must be proven from the statistical result from which the stopping criterion has been derived, hence the difficulty to come up with new and useful \Acp{SA}. 

Concentration inequalities are however a good source of theorems that can lead to meaningful stopping criteria. For instance, the NAS algorithm \cite{domingo2000madaboost} is a \Ac{SA} developed by \citeauthor{domingo2000madaboost} for bounded random variables with expected value $\Mean \neq 0$. It is a straightforward \Ac{SA} whose stopping criterion is of the form $|\Estimator{\Mean}_t| < c_t$, where $c_t = \sqrt{\frac{\log(t(t+1)/\ConfMargin)}{2t}}(1+1/\Precision)$ are parameters of the algorithm. 
The expressions for these parameters are derived from the Hoeffding's inequality \cite{hoeffding1994probability}.

The \EBStop algorithm \cite{mnih2008empirical} was introduced in 2008 by \citeauthor{mnih2008empirical} as an improvement of the NAS algorithm. Similarly to its predecessor, \EBStop builds a sequence of parameters $c_t$ as its stopping criterion. However, by exploiting the (empirical) Bernstein's inequality \cite{audibert2007tuning} instead of the Hoeffding's inequality, the variance of the random variable $X$ takes part in the computation of such parameters. 
Especially when the variance is significantly smaller than the range $R$ of the random variable, these parameters decrease much faster, therefore putting an end to the sampling process much sooner. 
For any fixed sequence $(d_t)_{t \in \Naturals}$ such that $\sum_{t=1}^{\infty}d_t \le \ConfMargin$, the parameters $c_t$ can be taken as $c_t = \Estimator{\sigma}_t \sqrt{\frac{2\log(3/d_t)}{t}} + \frac{3R\log(3/d_t)}{t}$, with $\Estimator{\sigma}_t$ being the sample standard deviation at step $t$. 
%
%
The \EBStop algorithm adds another improvement to the most basic version of the NAS algorithm. The stopping criterion is divided into a lower stopping criterion $(1+\Precision) \max\Set{0,\max_{1 \le s \le t}(|\Estimator{\Mean}_s| - c_s)}$ and to an upper stopping criterion $(1+\Precision) \min_{1 \le s \le t}(|\Estimator{\Mean}_s| - c_s)$, so that $X$ must not be supposed non-negative. 
The most upgraded version of the algorithm, called \EBGStop, also adopts a geometric sampling strategy, accumulating samples at an exponential rate $\beta$ rather than with a linear rate. The right choice of $\beta$ and additional countermeasures \cite{mnih2008empirical,audibert2007variance} allow for a speed-up of the algorithm without running the risk of taking more samples than needed. 

If $R > 0$ is the range of the random variable $X$, \citeauthor{mnih2008empirical} proved that the \EBStop algorithm will require a sample size smaller than a multiple of 
   $\max\Set{\frac{\sigma^2}{\Precision^2,\Mean^2},\frac{R}{\Precision|\Mean|}} \times \left(\log \frac{1}{\ConfMargin} + \log \frac{R}{\Precision|\Mean|}\right)$, 
which guarantees its (near-)optimality in a similar way to is main competitor: the \ApproxAlgo algorithm.

The \ApproxAlgo algorithm \cite{dagum2000optimal} is a \Ac{SA} in three steps, introduced in 2000 by \citeauthor{dagum2000optimal}\
It was built upon the theory of supermartingales and a generalized version of the zero-one estimator theorem. It can only be applied to any bounded and non-negative random variable $X$. \ApproxAlgo is significantly more complex than \EBStop. Actually, \ApproxAlgo can be seen as a relatively basic Monte-Carlo algorithm for its second and third steps, with the size of the required sample being computed indirectly with a \Ac{SA} during the first step. 
%
\ApproxAlgo first computes a $\left(\max\Set{\sqrt{\Precision}, \frac{1}{2}}, \frac{\ConfMargin}{3}\right)$-approximation $\tilde{\Mean}$ of $\Mean$, which is only used to compute a Monte-Carlo estimation $\tilde{\sigma}^2$ of $\sigma^2$, which is in turn exploited to derive a value $N = \max\Set{\tilde{\sigma}^2, \Precision \tilde{\Mean}} \frac{\log(\frac{1}{\ConfMargin})}{\Precision^2 \tilde{\Mean}^2}$ for the final sample size which guarantees that the final Monte-Carlo estimation $\Estimator{\Mean}$ is an \PrecConf-approximation $\Estimator{\Mean}$ of $\Mean$. 

While the hypothesis that $X$ is non-negative makes \ApproxAlgo a bit more restrictive than \EBGStop, it was proven to be fully optimal for that class of random variables. Namely, for any bounded and non-negative random variable $X$, \citeauthor{dagum2000optimal} showed that with probability $1-\ConfMargin$, \ApproxAlgo will require a sample size that is at most a multiple of $\max\Set{\sigma^2,\Precision \Mean} \times \frac{1}{\Precision^2 \Mean^2} \log(\frac{2}{\ConfMargin})$, while also proving that any \Ac{SA} designed for that class of random variables will always require with probability $1-\ConfMargin$ a sample size of at least a multiple of that exact quantity.

Contrary to the expression of optimality of \EBGStop, the expression of optimality of \ApproxAlgo does not involve the range of the random variable, which can be linked to the fact that while both algorithms exploit information about the variance, they do not do it in the same way. This hints at the possibility that even for non-negative bound random variables, for which both algorithm can be applied, \EBGStop can outperform \ApproxAlgo in practice.

==> 02-background.tex <==
%!TEX root = ./root.tex
In this section we introduce some key mathematical concepts and discuss the notion of $\PrecConf$-approximation algorithm. We then describe two optimal \Acp{SA} available from the literature.

We denote by $\Reals$, $\RealsGEZ$, $\Integers$, $\IntegersGEZ$ the sets of, respectively, real, non-negative real, integer, and non-negative integer numbers. Given sets $A$ an $B$, $A^B$ denotes the set of functions from $B$ to $A$. Finally, given a random variable $X$, we denote by $\Expectation(X)$ the expectation of $X$.


\AcronymReset{SA}%

\SectionInput
   {Unbiased estimators}
   {02-background-estimators.tex}

\SectionInput
   [sec:preliminaries:sa]
   {\Aclp{SA}}
   {02-background-stopping-algorithms.tex}



==> 03-formal-framework.tex <==
%!TEX root = ../root.tex
%
\Acp{CPS} are naturally modeled as dynamical systems (see, \eg \cite{sontag2013mathematical}).
Model-based verification of a \Ac{CPS} amounts to checking whether some system requirements are verified. 
%
Such a task thus requires three components: a model of the system, the set of possible \emph{operational scenarios} (\ie input time functions), and a formalization of the specification to be verified.

Due to their complexity and diversity, many different formal frameworks have been proposed to define models for \Acp{CPS}. State-based transition models, defined explicitly or through differential equations (with discrete or continuous time) are the most prevalent. 

In this article however, for the sake of generality, we abstract away from any specific formal framework for the definition of the system model and simply assume (along the lines of, \eg \cite{mancini2014anytime,mancini2016anytime,esposito2022estimation,esposito2022formal}) that our \emph{\Ac{SUV}} $\SUV$ is modeled (\cref{def:suv}) as a black-box input-output deterministic strictly causal dynamical system, which takes as input an \emph{operational scenario}, \ie a time function of both the controllable inputs and the other uncontrollable events $\SUV$ is subject to (\eg faults in sensors and actuators or changes in system parameters), and produces a time function of system outputs (called \emph{output function} or \emph{trajectory}).

\begin{definition}[\Acl{SUV} model]
    \label{def:suv}
    A \Acf{SUV} model $\SUV$ is a tuple $\SUVDef$ where:
    \begin{itemize}[compact]
        \item $\TimeSet$ is the \emph{time-set} ($\RealsGEZ$ or $\IntegersGEZ$ for continuous- and discrete-time systems, respectively, or an interval thereof);

        \item Sets $\InSpace$ and $\OutSpace$ are the \emph{input and output spaces}; 

        \item $\SimFun: \InSpace^{\TimeSet} \to \OutSpace^{\TimeSet}$ is the \emph{I/O} (or \emph{simulation}) \emph{function}. 
        For any \emph{input function} $\InFun \in \InSpace^{\TimeSet}$ (\emph{operational scenario}), $\SimFun(\InFun)$ denotes the \emph{output function} $\OutFun \in \OutSpace^{\TimeSet}$ of $\SUV$, defining the output $\OutFun(t)$ of $\SUV$ for each time point $t \in \TimeSet$, when the system is fed with $\InFun$.
    \end{itemize}

    With a small abuse of notation, we denote by $\SimFun(t; \InFun)$ the output of $\SUV$ at time point $t$ when fed with $\InFun$, \ie $\SimFun(\InFun)(t)$.

    A \emph{strictly causal} \Ac{SUV} model $\SUV$ is such that, for any $t \in \TimeSet$ and for any $\InFun_1, \InFun_2 \in \InSpace^{\TimeSet}$ such that $\InFun_1(t') = \InFun_2(t')$ for all $t' < t$, it holds $\SimFun(t; \InFun_1) = \SimFun(t; \InFun_2)$. 
\end{definition}



Models for \Acp{SUV} must therefore at the very least be executable (black box) models, with respect to discrete or continuous time, such that they output a unique output function (trajectory) for any given operational scenario.


The full set of operational scenarios of interest for a system (\ie those considered possible or on which the verification activity needs to focus), together with a probability measure of each scenario to materialize is collectively called the \emph{environment} of the \Ac{SUV} (\cref{def:environment}).
For practical reasons, we focus on \emph{finitely parameterizable} system environments, \ie environments whose scenarios can be modeled via a finite real- or discrete-valued parameter vector. 
We remind that a scenario encodes both user (controllable) inputs to the system and other uncontrollable events.

\begin{definition}[Stochastic system environment]
    \label{def:environment}
    Let $\SUV = \SUVDef$ be a \Ac{SUV} as in \cref{def:suv}. An environment $\Env = \EnvDef$ for $\SUV$ is defined by a set $\EnvInputSet \subseteq \InSpace^{\TimeSet}$ of scenarios and an associated probability distribution $\Prob : \EnvInputSet \to [0,1]$.     

    An environment is \emph{finitely parameterizable} if there exist a finite-dimension parameter vector space $\EnvInputSetParamSpace$ and a bijection between $\EnvInputSetParamSpace$ and $\EnvInputSet$.
\end{definition}

A metric \Ac{KPI} of the \Ac{SUV} is a function associating a real value to each system trajectory. 
With \cref{def:kpi} we limit ourselves to normalized \Acp{KPI}, that is \Acp{KPI} assuming values in interval $[0,1]$.

\begin{definition}[Normalized metric \Ac{KPI}]
    \label{def:kpi}
    A normalized metric \Ac{KPI} for \Ac{SUV} $\SUV$ is a function $\KPI: \OutSpace^{\TimeSet} \to [0,1]$.
\end{definition}

In order to ensure that also $\PrecConf$-approximation algorithms requiring \emph{bounded non-negative} random variables, such as \ApproxAlgo (see \cref{sec:preliminaries:sa}), can be exploited by \EAA, in the following we focus on model-based \Ac{SUV} verification problems where the property to be assessed is threshold-based (\cref{def:problem}):

\begin{definition}[Threshold-based verification problem]
    \label{def:problem}
    A threshold-based verification problem for a \Ac{SUV} model $\SUV = \SUVDef$, an environment $\Env = \EnvDef$, a threshold $\Threshold \in [0,1]$ and a normalized metric \Ac{KPI} $\KPI: \OutSpace^{\TimeSet} \to [0,1]$ consists of deciding whether $\Expectation_{\InFun \in \EnvInputSet}(\KPI(\SimFun(\InFun))) \leq \Threshold$, where the expected value is computed with respect to the probability distribution $\EnvProb$ of scenarios as defined in $\Env$.
\end{definition}

Any approximation algorithm which provides an unbiased $\PrecConf$-estimator for the expected value of a $[0,1]$-valued random variable can be applied to the binary random variable $X = (\SimFun(\EnvInputSet) \leq \Threshold)$ to offer a probabilistic answer to a threshold-based verification problem. 
%
Indeed, if an $\PrecConf$-approximation $\Estimator{\Mean}$ of $\Mean = \Expectation(\KPI(\SimFun(X))$ can be computed, then we know that, with probability at least $1-\ConfMargin$:
    $$
        \Mean(1 - \Precision) \leq 
            \Estimator{\Mean} \leq 
                \Mean (1 + \Precision).
    $$

Therefore:
    $$
        \frac{\Estimator{\Mean}}{1 + \Precision} \leq 
            \Mean \leq 
                \frac{\Estimator{\Mean}}{1 - \Precision}.
    $$

In conclusion, since $\frac{\Estimator{\Mean}}{1 - \Precision} \leq \Threshold$ implies that $\Mean \leq \Threshold$, it suffices to check whether:
\begin{equation}
    \label{eq:kpi:comparison}
    \frac{\Estimator{\Mean}}{1 - \Precision} - \Threshold \leq 0.
\end{equation}

If that inequality holds, then the requirement of the system associated with the threshold $\Threshold$ and the \Ac{KPI} $\KPI$ is successfully verified with a precision of $\Precision$ and a $1-\ConfMargin$ level of confidence.
%
A threshold-based verification problem with a lower bound threshold can be defined and solved in a very similar fashion.


==> 04-eaa-algo.tex <==
%!TEX root = ../root.tex
\begin{algorithm}[H]
    \caption{\Acs{EAA}}
    \label{algo:eaa}

    \KwIn: $\SUV$, \Ac{SUV} model\;
    \KwIn: $\Env$, stochastic environment\; 
    \KwIn: \AlgoVar{seed}, random seed\;
    \KwIn: $\Precision, \ConfMargin \in (0,1)$\;
    \KwIn: $\Algo_1, \ldots, \Algo_{\AlgoNb}$, set of $\PrecConf$-appr.\ algorithms\;

    \BlankLine
                
    initialize rnd scen.\ generator with $\Env$ and \AlgoVar{seed}\;
    initialize simulator with $\SUV$\; 
    initialize $\Algo_1, \ldots, \Algo_{\AlgoNb}$ with $\Precision$ and $\ConfMargin$%
        \nllabel{line:algo:eaa:sa-module:start}%
        \;
    
    \AlgoVarGets
        {$s_{1}, \ldots, s_{\AlgoNb}$}
        {initial states of $\Algo_1, \ldots, \Algo_{\AlgoNb}$}%
        \nllabel{line:algo:eaa:init}\;
    %with $\Precision$ and $\ConfMargin$\;

    %\AlgoVarGets{$t$}{0}\tcp*{number of generated samples}
    \While{\AlgoVar{true}}{%
        \nllabel{line:algo:eaa:loop}        
        \AlgoVarGets
            {$x$}
            {\AlgoFun{next\_sample()}}\;

        \For{$l$ \KwFrom 1 \KwTo $\AlgoNb$}{%
            \nllabel{line:algo:eaa:advance}
            \AlgoVarGets
                {$s_{l}$}
                {$\Fun{advance}_{\Algo_l}(s_{l}, x)$}
                \tcp*{feed $\Algo_l$ with $x$}%
                %\;

            \If{$\Algo_{l}$ has reached its stopping cond.}{%
                \Return{$\Estimator{\Mean}_{l}$}%
                \tcp*{the estimated mean from $\Algo_{l}$}
                \nllabel{line:algo:eaa:stop}%
                \nllabel{line:algo:eaa:sa-module:end}%
            }
        }
    }    

\BlankLine

\AlgoFunction{next\_sample()}{%
    \AlgoVarGets
        {$\InFun$}
        {generate next rnd scenario}\;
    \AlgoVarGets
        {$x$}
        {simulate $\InFun$}%
            \tcp*{obtain \Ac{KPI} value (sample)}%
    \Return{$x$}\;
}
\end{algorithm}

==> 04-eaa.tex <==
%!TEX root = ./root.tex
As explained in \cref{sec:formal-framework}, any adaptive \Ac{SA} which computes an $\PrecConf$-approximation of the expected value of a $[0,1]$-valued random variable provides a \Ac{SMC} method to solve threshold-based verification problems. 
%
Moreover, as discussed in \cref{sec:background}, the number of samples \emph{actually} needed by any given \Ac{SA} to converge on a given verification task depends not only on the requested properties of the approximation, but also on statistical properties of the \Ac{KPI} to be approximated, which are typically unknown in advance.
%
In settings, such as \Ac{SMC} model-based verification of \Acp{CPS} where generating samples of the system \Ac{KPI} of interest is particularly expensive, because it requires numerical simulation of the \Ac{CPS} model, using a single \Ac{SA} to perform \Ac{SMC} might result in an unnecessary large number of samples to be generated. This is true also for those \Acp{SA} proved to be optimal like \ApproxAlgo, since optimality in the number of required samples is guaranteed only probabilistically and up to a multiplicative factor.

In a similar fashion to AI-based techniques such as \emph{ensemble learning} methods \cite{sagi2018ensemble,dong2020survey}, 
we propose a general procedure, named \Ac{EAA}, that exploits a finite set $\Algo_1, \ldots, \Algo_{\AlgoNb}$ of different $\PrecConf$-approximation algorithms. 

The $\EAA$ algorithm (see \cref{fig:eaa} for a conceptual high-level view and pseudocode) first initializes the states of all the algorithms in the ensemble (line~\ref{line:algo:eaa:init}). 
Then, it repeatedly generates samples of random variable $X$. 
In our case, this means to generate a random scenario $\InFun$ for the \Ac{SUV}
(line~\ref{line:algo:eaa:loop}), to simulate the \Ac{SUV} model on it, and to compute the associated value ($x$) of the \Ac{KPI} of interest.
Each sample $x$ is then used to feed and advance \emph{all} algorithms of the ensemble (line~\ref{line:algo:eaa:advance}) \emph{by one step only} (\ie processing only $x$). This is done by functions $\AlgoFun{advance}_{\Algo_{l}}$() ($l \in [1, \AlgoNb]$).

As soon as one of the algorithms (say $\Algo_{l}$) reaches its termination condition, \EAA stops and returns the approximation $\Estimator{\Mean_l}$ provided by $\Algo_{l}$ (line~\ref{line:algo:eaa:stop}), which is a valid $\PrecConf$-approximation of the true mean $\Mean$ of the value of the \Ac{KPI} of interest. Value $\Estimator{\Mean_l}$ is then used to answer the threshold-based verification problem, by checking whether \cref{eq:kpi:comparison} holds.

Since the procedure terminates as soon as the first algorithm in the ensemble, say $\Algo_{l}$, reaches \emph{its own} stopping criterion, the number of samples required by \EAA is always the \emph{minimum} number of samples that would have been required by each algorithm in the ensemble if it were run alone.

The design of \EAA revolves around proper subroutines that advance each algorithm in the ensemble by one step (\ie processing just one sample) at the time and manipulate the algorithm persistent state appropriately. 
Namely, each $\AlgoFun{advance}_{\Algo_{l}}()$ subroutine: 
(a)~takes as input the current state $s_i$ of algorithm $\Algo_{l}$ and a new sample $x$;
(b)~processes $x$ by advancing the algorithm state into $s_{l}'$;
(c)~returns the resulting state $s_{l}'$.
Such subroutines can be easily written by refactoring any approximation algorithm.
%
In our implementation (see \cref{sec:expres}) we selected two of the most widely known algorithms known to be optimal or quasi-optimal (probabilistically and up to a multiplicative factor): \EBGStop and \ApproxAlgo, already described in \cref{sec:preliminaries:sa}. 
%
Advancing each algorithm in the ensemble only requires a few algebraic operations. Thus, the computational overhead of advancing multiple algorithms in the ensemble is expected to be \emph{negligible} with respect to the (much longer) time to perform simulations of the \Ac{SUV} model to produce each sample. This expectation will be shown correct in \cref{sec:expres:sampler}.

\begin{figure}
		\centering
		\includegraphics[scale=0.8]{architecture.pdf}

		\caption{Conceptual view of \Ac{EAA} (sequential reference architecture).}	
		\label{fig:eaa}

	 	\Input{04-eaa-algo.tex}
\end{figure}



==> 05-hpc-eaa-algo.tex <==
%!TEX root = ../root.tex
\begin{algorithm}[H]%[ht]
    \AcronymUsed{HPC-EAA}%
    \caption{\Acf{sampler}}
    \label{algo:sampler}

    \KwGlobal $i = 0$\tcp*{id of the next sample to be produced}
    \KwGlobal $j = 0$\tcp*{id of the next sample to be consumed by \Ac{EAA}}
    \KwGlobal $\AlgoVar{avail\_sims} = \emptyset$%        
        \tcp*{queue of avail.\ simulators}

    \KwGlobal $\AlgoVar{samples} = \emptyset$%
        \tcp*{map: \emph{sample id} $\mapsto$ \emph{\Ac{KPI} value}}

    \KwParam $\SimNb$%
        \tcp*{number of available simulators}

    \BlankLine

    \KwFunction \AlgoFun{initialize($\SUV$, $\Env$, \AlgoVar{seed})}\NoBeginEnd{%
        \nllabel{algo:sampler:init}
        initialize random generator with $\Env$ and \AlgoVar{seed}\;

        initialize the $\SimNb$ available simulators with $\SUV$ and enqueue them all to \AlgoVar{avail\_sims}%
        \nllabel{algo:sampler:avail_sims:init}%
        \;

        start process \AlgoFun{generate\_samples()}\;
    }

    \KwProcess \AlgoFun{generate\_samples()}\NoBeginEnd{%
        \nllabel{algo:sampler:generate}
        \tcp{continuous process}
        \While{$\lnot$ halt requested}{
            \AlgoVarGets
                {$\InFun$}
                {generate rnd scenario}\;                    

            \AlgoVarGets
                {sim}
                {dequeue from \AlgoVar{avail\_sims}}%
                \nllabel{algo:sampler:avail_sims:wait}%
                \tcp*{wait if queue is empty}

            send $(i, \InFun)$ to \AlgoVar{sim} for simulation and \Ac{KPI} evaluation\;

            \AlgoVarIncr{$i$}\;
         }
    }

    \KwFunction \AlgoFun{sample\_produced(\AlgoVar{sim}, $i$, $x$)}\NoBeginEnd{%
        \nllabel{algo:sampler:sample_produced}%
        \tcp{called by simulator \AlgoVar{sim} when evaluation of scenario $i$ is completed (\Ac{KPI} value is $x$)}
        add $(i \mapsto x)$ to \AlgoVar{samples}%
            \tcp*{wait if map is full}
        enqueue \AlgoVar{sim} to \AlgoVar{avail\_sims}\;
    }

    \KwFunction \AlgoFun{next\_sample()}\NoBeginEnd{%
        \nllabel{algo:sampler:next_sample}%
        \tcp{called by \EAA}

        \AlgoVarGets
            {$x$}
            {\AlgoVar{samples[$j$]}}%
            \tcp*{wait if not yet available}

        free-up \AlgoVar{samples[$j$]}\;

        \AlgoVarIncr{$j$}\;

        \Return{$x$}\;
    }
\end{algorithm}    
 

==> 05-hpc-eaa.tex <==
%!TEX root = ./root.tex
%
\Ac{SMC}-based verification often requires a huge number of samples, that is, computer simulations of the \Ac{CPS} model.
%
As discussed in \cref{sec:introduction}, this is particularly the case for complex systems. 
%
For example, verifying the properties defined in \cref{sec:expres:case-studies} on our case studies required up to more than 100 million samples.

While \EAA allows us to stop the verification process as soon as the first algorithm of the ensemble reaches its termination condition, it does not address the second major bottleneck of model-based \Ac{CPS} verification via \Ac{SMC}: the rate at which samples are provided to the approximation algorithm. 
%
For our case studies, generating a single sample took, on average, from $0.1$ to several seconds, depending on the model.
As a consequence, the verification activities we performed (see \cref{sec:expres}) would have required up to many years for \EAA to terminate if conducted na{\"i}vely.

In this section we outline our approach to exploit \Ac{HPC} platforms to effectively and efficiently speed-up the generation of samples to be provided to \EAA.

Our overall architecture is shown in \cref{fig:parallel-architecture}. It is designed to run on a possibly very large \Ac{HPC} infrastructure, and includes: 
a multi-process or multi-threaded module devoted at advancing the \Acp{SA} of the ensemble one sample at a time (lines~\ref{line:algo:eaa:sa-module:start}--\ref{line:algo:eaa:sa-module:end} of \cref{algo:eaa}); 
$\SimNb$ instances (with $\SimNb$ which can be very large) of a simulation module, each one running an identical copy of a simulator of the \Ac{SUV} model; 
one multi-process or multi-threaded module hosting a service, named \Ac{sampler}, devoted to the generation of random scenarios and the delegation of the simulation of each of them to one of the $\SimNb$ available parallel simulators.
%
Since the latter service runs asynchronously with respect to the \Acp{SA}, the overall architecture implements an instance of the \emph{producer-consumer paradigm}.

\begin{figure}
	\IncludeGraphics[scale=0.8]{parallel-architecture.pdf}
	\caption{\Ac{HPC-EAA}: high-level parallel architecture.}
	\label{fig:parallel-architecture}

	\bigskip
	\input{05-hpc-eaa-algo.tex}
\end{figure}

The exact operation of \Ac{sampler} is described in details by \cref{algo:sampler}.
%
First, function \AlgoVar{initialize}() (line~\ref{algo:sampler:init}) initializes \Ac{sampler} with the given \Ac{SUV} model $\SUV$, its environment $\Env$, and a random seed to generate scenarios from $\Env$.
This function instantiates the $\SimNb$ simulators with identical copies of $\SUV$ and initializes the random scenario generator.
Note that, since the environment is finitely parametrizable, scenario generation reduces to generating pseudorandom numerical vectors within some bounded finite-dimensional domain (see \cref{def:environment}). 
Then, function \AlgoVar{initialize}() starts process (or thread) \AlgoFun{generate\_samples()} and returns immediately.

Process \AlgoFun{generate\_samples()} (line~\ref{algo:sampler:generate}) continuously generates (see bullet point 1 in \cref{fig:parallel-architecture}) a random scenario $\InFun$ from the system stochastic environment, retrieves (\emph{dequeues}) a simulator \AlgoVar{sim} from the queue of idle simulators (bullet point 2), and delegates to \AlgoVar{sim} the two tasks of simulating $\SUV$ under scenario $\InFun$ and of computing the value of the \Ac{KPI} of interest.
The queue of idle simulators is initially filled with identifiers of all the available simulators (line~\ref{algo:sampler:avail_sims:init}). If found empty, the process waits (\emph{blocking dequeue} operation) for a simulator to become idle (line~\ref{algo:sampler:avail_sims:wait}).
%
Each scenario is identified by a progressive number (integer $i$ in the pseudocode). 

Whenever a simulator terminates its task on scenario $i$, having computed value $x$ for the \Ac{KPI} of interest, it calls function \AlgoFun{sample\_produced}() of \Ac{sampler}. 
This function (line~\ref{algo:sampler:sample_produced} and bullet point 3 in the figure) inserts entry $i \mapsto x$ in the map \AlgoVar{samples}, thus storing the value of the system \Ac{KPI} on scenario $i$ (this corresponds to the \emph{produce} step in the producer-consumer paradigm), and the simulator is added to the queue of idle simulators, signalling that it is ready to receive new simulation requests.
To prevent memory explosion, map \AlgoVar{samples} has a maximum capacity. If the map is full, the insertion of the new sample blocks until an entry is removed.

The module running the \Acp{SA} continuously (and asynchronously) requests samples from \Ac{sampler} by calling function \AlgoFun{next\_sample()} (this corresponds to the \emph{consume} step in the producer-consumer paradigm). 
This function (line~\ref{algo:sampler:next_sample} and bullet point 4 in the figure) returns the \Ac{KPI} value associated to scenario with id $j$ in the map \AlgoVar{samples} and waits in case such an entry does not (yet) exist (because not yet computed). 
Before returning, this function frees-up memory by removing from map \AlgoVar{samples} the entry associated to scenario $j$ and increments $j$, which becomes the id of the next sample to be provided to the \Acp{SA}.

It is worth noting that \Ac{sampler} provides the \Acp{SA} with the \emph{very same} sequence of samples that would be produced with the basic (purely sequential) architecture of \cref{fig:eaa}, if run with the same random seed. In other words, the order of the scenarios generated is \emph{independent} of the number $\SimNb$ of simulators. Thus, increasing $\SimNb$ will have no other effect than increasing the rate at which the samples are made available to \Acp{SA}, hence reducing the total completion time. 
In this way, we avoid any bias in the (pseudo-)randomness of the samples and so in the final result of the approximation.



==> 06-experiments-case-studies-alma.tex <==
%!TEX root = ../../../root.tex
\begin{Section}{System model}
    The \Ac{ALMA} model defines the logic of the phase-plane control algorithm for the autopilot program of the lunar module used in the Apollo 11 mission. This model has been extensively used in the literature on simulation-based verification (see, \eg \cite{mancini2021any,mancini2021checking} and citations therein).

    The system is equipped with 3 sensors (yaw, roll, pitch) and 16 reaction jets that actuate a rotation over one or more axes. In every space mission, \ie in every system simulation, the controller takes as input a request to change the module's attitude and computes which reaction jets need to be activated to achieve the desired rotation and stabilize the system over the new current attitude. 
\end{Section}



\begin{Section}{Environment}
    We modeled a stochastic environment where temporary faults may occur on yaw, pitch and roll sensors, similarly to what we did for the \Ac{FCS} model. 
    For this model, a fault corresponds to the injection of white noise to one of sensor signals. 
    Analogously to the \Ac{FCS} model, the occurrences of the faults are chosen according to an exponential distribution whose mean corresponds to a \Ac{MTBF} of $\Pretty[s]{4}$. 
    Similarly, fault recovery happen after a duration once again determined by an exponential distribution with a mean of \Pretty[s]{1}.
\end{Section}



\begin{Section}{Property to be verified}
    We designed a system-level requirement that quantifies the outcome of a given space mission in terms of the average module's attitude error over the entire simulation. 
    To define such an error, we first have to define the attitude error indicators for each axis. For each axis $s$, if $a_s(t)$ and $R_s$ denote the current and target attitudes at time $t$ along $s$, respectively, we define the attitude error $e_s$ at time $t$ as follows:
    %
    \begin{equation*}
        e_s(t) = |a_s(t) - R_s|
    \end{equation*}
    %
    that is, the absolute difference between the target and the current attitudes of the lunar module along axis $s$. 
    Since the rotation request is over one or more axes, we define the \emph{Attitude Module Error} (AME) at time $t$ as follows:
    %
    \begin{equation*}
        \Fun{AME}(t) = \max\Set{e_y(t), e_p(t), e_r(t)}
    \end{equation*}
    %
    where the $e_y(t)$, $e_p(t)$, and  $e_r(t)$ are, respectively, the attitude errors on the yaw, pitch and roll axes at time $t$.
    %
    Our final \Ac{KPI} is thus the \emph{Normalised Mean Attitude Module Error} at time $t$, defined as:
    %
    \begin{equation*}
        \Fun{NMAME}(t) = 
            \frac{1}{2\pi t} 
            \int_0^t \Fun{AME}(\tau) \Fun{d}(\tau)
    \end{equation*}
    %
    where $2\pi$ is a normalization factor, since a rotation along a given axis ranges in $[0, 2\pi]$.

    Similarly to the \Ac{AT} and the \Ac{FCS} models, the goal of our experiment is to verify whether $\Expectation(\Fun{NMAME}(\Horizon)) \leq \Threshold$ for some threshold.
    %
    We set $\Horizon = \Pretty[s]{60}$ and $\Threshold = 0.5\%$. 
    Note that greater values for $\Threshold$ systematically lead to system mission failures.
\end{Section}




==> 06-experiments-case-studies-at.tex <==
%!TEX root = ../../../root.tex
%
\begin{Section}{System model}
	The \Ac{AT} model defines a typical automotive drivetrain. 
	Non-linear ordinary differential equations are used to specify the engine dynamics, the four-speed automatic transmission and the vehicle dynamics. 
	The model has two inputs, the throttle opening (expressed in percentage) and the brake torque (expressed in ft-lb), and two outputs, the engine speed (in RPM) and the vehicle speed (in mph). 
	%
	The throttle opening delineates the accelerating dynamics, whereas the brake torque represents the braking dynamics of the vehicle. 

	In the literature, the \Ac{AT} system has been extensively used for search-based falsification purposes (see, \eg \cite{abbas2013probabilistic, hoxha2018mining, dokhanchi2015requirements}) and benchmarks (\eg \cite{hoxha2014benchmarks, ernst2022arch}), especially when the design of input trajectories has a strong impact on the verification (see, \eg \cite{barbot2020falsification}). 
\end{Section}

\begin{Section}{Environment}
	We modeled a stochastic environment for the system that generates disturbances as input time functions for the \Ac{SUV} model. 
	In our setting, the brake is always set to 0, whereas the throttle presents a fixed average value $\mu_{d}$ that is perturbed with a given variance $\sigma^2_{d}$, \ie the values are sampled from a normal distribution $N(\mu_{d}, \sigma^2_{d})$ truncated within $[0, 100]$.
	%
	We set $\mu_d=40$ and $\sigma^2_d=20$ for the truncated normal distribution, thus modeling a varying accelerating dynamics.
\end{Section}

\begin{Section}{Property to be verified}
	In the context of search-based falsification, a typical system-level specification requires that the engine and vehicle speeds do not exceed given safety thresholds for the whole simulation duration. 
	Therefore, we designed a (metric) safety property which quantifies how much time the engine and the vehicle speeds spend above such thresholds.

	To define our system-level requirement, we first have to define the maximum time window during which any of the two speed is above its thresholds. 
	We define the \emph{Max Time Speed} (MTS) and the \emph{Max Time Engine} (MTE) at time $t$ as:
	%
	\begin{align*}
		\Fun{MTS}(t) = 
			& \max\Set{t_2 - t_1 
				~\mid~ 0 \leq t_1 \leq t_2 \leq t \wedge 
					( \forall t' \in [t_1, t_2] : \Fun{speed}(t') > M_{s} )
			}  
		\\
		\Fun{MTE}(t) = 
			& \max\Set{t_2 - t_1 
				~\mid~ 0 \leq t_1 \leq t_2 \leq t \wedge 
					( \forall t' \in [t_1, t_2] : \Fun{engineRPM}(t') > M_{e})
			}
	\end{align*}
	%
	where $\Fun{speed}(t)$ and $\Fun{engineRPM}(t)$ are the values of the vehicle and engine speeds at time $t$, whilst $M_{s}$ and $M_{e}$ are the respective maximum safe values. 
	%
	The \emph{Max Time Violation} at time $t$ is then defined as:

	\begin{equation*}
		\Fun{MTV}(t) = \frac{\max\Set{\Fun{MTS}(t), \Fun{MTE}(t)}}{\Horizon}
	\end{equation*}
	%
	where $\Horizon$ is the simulation time horizon. 

	The verification activity aims to establish whether $\Expectation(\Fun{MTV}(\Horizon)) \leq \Threshold$ for some threshold.
	%
	We set $M_{s} = 4000$ RPM and $M_{e} = 120$ RPM (according to previous work, see, \eg \cite{fan2017dryvr,claessen2018using}), 
	$\Horizon = \Pretty[s]{1800}$ (\ie $\Pretty[minutes]{30}$ of system simulation time), and $\Threshold = 5\%$, so to assess whether the system violates the desired specification for any time window longer than $5\%$ of the time.
\end{Section}


==> 06-experiments-case-studies-fcs.tex <==
%!TEX root = ../../../root.tex
\begin{Section}{System model}
	The \Ac{FCS} model represents a control system for a fault-tolerant gasoline engine that is expected to accept up to one sensor fault, and has been widely used as a benchmark of various simulation-based verification approaches (see, \eg \cite{zuliani2010bayesian,mancini2013system,hoxha2014benchmarks,mancini2021any,mancini2021checking} and citations therein).  

	The system has four sensors: the \emph{Throttle Position} (TP), \emph{Engine Speed} (ES), \emph{Exhaust Gas Oxygen} (EGO) and \emph{Manifold Air Pressure} (MAP). 
	%
	The TP and ES sensors provide the current air throttle position and the engine speed to the engine controller. 
	The EGO sensor reads the current oxygen level in the engine's exhaust gas to adapt the fuel supply, whereas the MAP sensor reads the suction pressure of the airflow at the engine's intake manifold. 

	The model outputs the following two quantities: the \emph{air-fuel ratio}, that is, the ratio between the air mass flow rate computed by the intake manifold and the fuel mass flow rate pumped by the injectors, and the \emph{fuel flow rate} itself. 

	The system aims at keeping the air-fuel ratio close to the stoichiometric (ideal) value of \Pretty{14.6} since it is a good compromise between power, fuel economy and emissions.
	%
	However, this requirement becomes more challenging to meet in the presence of sensor faults. In particular, when a fault on a single sensor is detected, the system modifies its behavior by operating the engine with a higher fuel rate. In case of two or more sensor faults, the system shuts down the engine.
\end{Section}



\begin{Section}{Environment}
	We modeled a stochastic environment for the system where temporary faults may occur on the ES, EGO and MAP sensors. 
	Finite state machines (with Stateflow charts) were used to simulate fault injections and the subsequent recovery operations, similarly to, \eg \cite{zuliani2010bayesian,hoxha2014benchmarks}. 
	Each finite state machine injects faults on a given sensor according to an exponential distribution whose mean corresponds to the \Ac{MTBF}. Similarly, fault recovery operations occur after a time window whose length is randomly chosen according to an exponential distribution having a mean of \Pretty[s]{1}.
	%
	We set the \Ac{MTBF} values for the EGO, ES, and MAP to $\Pretty[s]{3}$, $\Pretty[s]{7}$ and $\Pretty[s]{8}$ respectively, which is the configuration used in \cite{zuliani2010bayesian} for verification purposes.
\end{Section}


\begin{Section}{Property to be verified}
	We experimented with one of the key system-level specifications for this model (see, \eg \cite{mancini2013system,mancini2021any,mancini2021checking}), that is establishing whether the fuel flow rate is identically zero for too long time. 
	%
	Therefore, we designed a \Ac{KPI} which outputs the (ratio of the) length of the longest time window during which the fuel flow rate is identically equal to zero. 
	%	
	%
	We define \emph{Max Time Fuel} (MTF) at time $t \geq \Pretty[s]{5}$ as follows (the first \Pretty[s]{5} of each trajectory have been ignored to allow for the initial setup of the system): 

	\begin{equation*}
		\Fun{MTF}(t)=
			\frac
				{ \max\Set{
							t_2 - t_1 
							~\mid~ 
							5 \leq t_1 \leq t_2 \leq t \wedge 
							( \forall t' \in [t_1, t_2] :
								\Fun{fuel}(t') = 0
							)
					}
				}
				{\Horizon - 5}
	\end{equation*}

	The goal of the verification is to establish whether $\Expectation(\Fun{MTF}(\Horizon)) \leq \Threshold$ for some threshold.
	%
	We set $\Horizon = \Pretty[s]{105}$ and $\Threshold = 1\%$, so to assess whether the fuel flow rate is identically zero for more than $1\%$ time on average. 
\end{Section}


==> 06-experiments-case-studies.tex <==
%!TEX root = ../../root.tex
%
\AcronymReset{AT}
\AcronymReset{FCS}
\AcronymReset{ALMA}
Our case studies were realized with three Simulink/Stateflow models of industry-scale systems, namely: \Ac{AT} \cite{AT}, \Ac{FCS} \cite{FCS} and \Ac{ALMA} \cite{ALMA}. 
These models have already been profusely studied in the literature, see, \eg \cite{mancini2021any,mancini2021checking,mancini2013system,zuliani2010bayesian,mancini2014anytime,mancini2017minimising,mancini2016sylvaas,hoxha2014benchmarks,abbas2013probabilistic,barbot2020falsification}.


\SectionInput
	{\Acf{AT}}
	{06-experiments-case-studies-at.tex}

\SectionInput
	{\Acf{FCS}}
	{06-experiments-case-studies-fcs.tex}

\SectionInput
	{\Acf{ALMA}}
	{06-experiments-case-studies-alma.tex}


==> 06-experiments-implementation.tex <==
%!TEX root = ../../root.tex
We implemented our production software using Python and Cython, and exploited the \Ac{MPI} standard \cite{gropp1999using} to allow communication between processes.

The overall architecture has been explicitly designed to be run on an a \Ac{HPC} infrastructure of networked computational nodes, and reflects that of \cref{fig:parallel-architecture} with some caveats to boost performance. 
The \Acp{SA} and \Ac{sampler} modules of \cref{fig:parallel-architecture} have been implemented as concurrent threads of a process named \Ac{HPC-EAA}, while the $\SimNb$ simulators have been deployed as independent processes on $\SimNb$ additional computational nodes.
%
\Ac{HPC-EAA} runs various parallel threads: one devoted to the advancement of each \Ac{SA}, one devoted to the generation of random scenarios and their delegation to an available simulator taken from the queue, and one devoted to process the receiving queue of samples and to populate map \AlgoFun{samples}. The use of such a thread-based implementation for the \Acp{SA} and \Ac{sampler} modules limits the use of the network to the communication with the simulators.


==> 06-experiments-results-ensemble.tex <==
%!TEX root = ../../../root.tex
%
To evaluate the benefit of using an ensemble of \Acp{SA}, for each case study we repeated our experiment 10 times. In each of them, we fed the \Acp{SA} module with one of the 10 random sequences of \Ac{iid} samples computed in advance for that model, as described in \cref{sec:expres:setting}, and computed the number of samples required by each of the two \Acp{SA} of the ensemble to converge. 
The number of samples required by \EAA is then the minimum of the two.

\Cref{fig:expres:eaa} (top) shows, for each case study and for each of the 10 random sequences of samples, the number of samples required by \Ac{EAA} to converge, for each value of $\Precision$ and $\ConfMargin$. 

Similarly, \cref{fig:expres:eaa} (bottom) shows the difference in the number of samples between the two \Acp{SA}, which is also the saving achieved if using \EAA, when compared to using the slowest algorithm only, together with information about which of the two \Acp{SA} terminated first, and so was responsible for producing the sought $\PrecConf$-approximation.
%
From the figure is clearly emerges how using \Ac{EAA} is a particularly effective way to keep the number of required samples to a minimum.
Indeed, our experiments show that \Ac{EAA} may require up to 
	\DataGet{exps/eaa/samples reduction/max} 
fewer samples when compared to using a single algorithm, with relative reductions as large as \DataGet{exps/eaa/samples reduction/max/perc}.

Predicting which algorithm of the ensemble will terminate first is a difficult task \emph{a priori}, since it depends not only on $\Precision$, $\ConfMargin$ and on statistical properties of the \Ac{KPI} of interest (with the latter being typically unknown in advance), but may also be influenced by the actual random sequence of \Ac{iid} samples (\ie on the seed of the pseudorandom number generator). 
The results for the \Ac{ALMA} case study (see \cref{fig:expres:eaa}, bottom) are a good illustration of that phenomenon. 
\EAA also provides a stabilizing effect in this regard.
Indeed, differently from what emerges in \cref{fig:expres:eaa} (bottom), the curves in \cref{fig:expres:eaa} (top) regarding the same case study and the same value for $\ConfMargin$ (but generated using different random sequences of samples) overlap with each other almost perfectly.



\begin{figure}
	\scriptsize
	\addtolength{\abovecaptionskip}{-3pt}
	\renewcommand{\tabularxcolumn}[1]{m{#1}}
	%
	\newcolumntype{Y}{>{\centering\arraybackslash}X}
	\renewcommand{\tabcolsep}{2pt}
	\newcommand
		{\TopLeftYLabel}
		{\rotatebox{90}{%
			\# samples (log scale)
		}}	
	\def\tmpSavingString{%
		{\ApproxAlgo} saving 
			\hspace{5ex}
		{\EBGStop} saving%
	}%
	\newcommand
		{\BottomLeftYLabel}
		{\raisebox{3ex}{\rotatebox{90}{%		
			\begin{minipage}{\widthof{~~\tmpSavingString~~}}%
				\begin{center}
					\# samples (log-scale)
					\par
					\tmpSavingString	
				\end{center}
			\end{minipage}%
		}}}
	\newcommand
		{\XLabel}
		{\ensuremath{\Precision~(\times 10^{-2})}}
	\begin{tabularx}
		{\linewidth}
		{
			m{4ex}
			*{3}{Y}
		}
		  % empty
		& \Acs{AT}
		& \Acs{FCS}
		& \Acs{ALMA}
		\\[1ex]		  
		  \TopLeftYLabel
		& \includegraphics
			[width=\linewidth]
			{sample_size_AT.pdf}	
		& \includegraphics
			[width=\linewidth]
			{sample_size_FCS.pdf}	
		& \includegraphics
			[width=\linewidth]
			{sample_size_ALMA.pdf}
		\\
		  \BottomLeftYLabel
		& \includegraphics
			[width=\linewidth]
			{sample_saving_AT.pdf}	
		& \includegraphics
			[width=\linewidth]
			{sample_saving_FCS.pdf}	
		& \includegraphics
			[width=\linewidth]
			{sample_saving_ALMA.pdf}		
		\\[-1ex]
		  % empty
		& \XLabel
		& \XLabel
		& \XLabel
	\end{tabularx}
	
	\caption{%
		Top: number of samples (vertical log-scale axis) required by \EAA to converge in each of the 10 experiments, for various values of $\Precision$ and $\ConfMargin$.
		%
		Bottom: savings in the number of samples achieved by \EAA in each setting wrt.\ the algorithm requiring most samples. 
	}
	\label{fig:expres:eaa}
\end{figure}


==> 06-experiments-results-sampler.tex <==
%!TEX root = ../../../root.tex
%
Here, we analyze the impact of deploying \Ac{sampler} on a parallel \Ac{HPC} infrastructure.
%
Namely, in \cref{fig:expres:speeds} (a) we show an estimation (with the method outlined in \cref{sec:expres:setting}) of the maximum rate $\RateSampler{\SimNb}$ of sample production when varying the number $\SimNb$ of available simulators. 
For each value of $\SimNb$, $\RateSampler{\SimNb}$ has been obtained by replacing the \Acp{SA} module with a simple loop requesting (and just throwing away) 1 million samples from \Ac{sampler} governing $\SimNb$ parallel simulators. 
Hence, these values are the highest sample production rates actually achievable by \Ac{sampler} on our infrastructure when using $\SimNb$ simulators of the given model.
\Cref{fig:expres:speeds} (a) shows that all $\RateSampler{\SimNb}$ are practically linear with respect to $\SimNb$, with a maximum deviation between the actual and the ideal (linear) rates $< 0.1\%$.

In \cref{fig:expres:speeds} (b) we show again the three values for $\RateSampler{\SimNb}$, this time using a logarithmic Y axis and along with the maximum rate $\RateEAA$ of consumption of samples by the \Acp{SA} module. 
%
Rate $\RateEAA$ has been obtained by replacing \Ac{sampler} and the controlled simulators by a simple pseudorandom generator feeding the \Acp{SA} module with numerical values in $[0,1]$, and measuring how long it took to consume 1 million of such samples. 
This value is thus the lowest rate of samples that \Ac{sampler} would need to provide to the \Acp{SA} module (running on our infrastructure) to allow the latter to advance at full speed.

From \cref{fig:expres:speeds} (b) it clearly emerges that $\RateEAA$ is always several orders of magnitude higher than all $\RateSampler{\SimNb}$ (even when the largest number of simulators, $\SimNb = 2048$, is deployed, in which case is still more than $100$ times larger). 
%
This means that the \Acp{SA} module would spend almost its entire time waiting for \Ac{sampler} to produce the requested samples. 
Hence, an increase in the number of simulators is expected to result in an essentially proportional reduction in the completion time of the overall parallel tool.
In order words, we expect our architecture to show an efficiency very close to $100\%$ even when a large number of simulators are used. This suggests that adding more algorithms to the ensemble of \Acp{SA} would not introduce any noticeable computational overhead, but could help in reducing the number of required samples for \Ac{EAA} if those additional algorithms happen to benefit from the statistical properties of the system \Ac{KPI}.

\begin{figure}
        \vspace{0pt}
	\begin{minipage}[t]{0.49\linewidth}
            \vspace{-2.5pt}
		\includegraphics
			[width=\linewidth]
			{parallel_prod_cons_speed_eval_linear.pdf}

		\caption*{(a)}
	\end{minipage}
	\hfill
	\begin{minipage}[t]{0.49\linewidth}
            \vspace{0pt}
		\includegraphics
			[width=\linewidth]
			{parallel_prod_cons_speed_eval_log.pdf}

		\caption*{(b)}
	\end{minipage}

	\caption{%
		(a)~Rates of sample production by \Ac{sampler} ($\RateSampler{\SimNb}$), for various numbers of available simulators (the grey curves are the \emph{straight} lines passing by the two left-most points of each data series, and show the almost perfect linearity of the sample production rates wrt.\ $\SimNb$).
		\\
		(b)~Comparison (log-scale Y axis) among the sample consumption rate by \Ac{EAA} ($\RateEAA$) and the sample production rates by \Ac{sampler} from Figure~(a).
	}
	\label{fig:expres:speeds}
\end{figure}




==> 06-experiments-results-scalability.tex <==
%!TEX root = ../../../root.tex
%
To confirm the above, here we describe a performance scalability analysis of our parallel implementation, estimating (again with the method outlined in \cref{sec:expres:setting}) its completion time if deployed on fully-reserved \Ac{HPC} infrastructures of various sizes.

\Cref{fig:expres:scalability} shows the time that our tool would require to terminate on each of the 10 experiments for each case study, as a function of $\Precision$, $\ConfMargin$, and the number $\SimNb$ of parallel simulators (notice the left log-scale Y axes). 
Each figure shows, for each value of $\ConfMargin$, the average completion time of the parallelization, with error bars indicating the minimum and the maximum values among the 10 experiments (error bars are often very tiny and barely visible, and this shows again the stability of the algorithm performance with respect to the random sequence of samples).
As expected, all the curves are qualitatively very similar, modulo the time reductions essentially proportional to $\SimNb$. 

Each plot in \cref{fig:expres:scalability} also shows (see the curves at the top, to be read against the linear-scaled right Y axes) the average estimated efficiency of the parallelization (with error bars indicating the minimum and the maximum values among the 10 experiments). 
The efficiency of the parallel computation involving $\SimNb$ simulators is computed, as usual, as $\frac{t_1}{\SimNb \times t_{\SimNb}}$, where, in our case, $t_{\SimNb}$ is the (estimated) time of the computation when using $\SimNb$ simulators and $t_1$ is the time of \emph{same} computation (\ie same values for $\Precision$, $\ConfMargin$ and same random sequence of samples) when using a single simulator.

As expected, the estimated efficiency always sticks to $\sim 100\%$, except when the number of simulators (hence, the size of the envisioned \Ac{HPC} infrastructure) is too large for the problem at hand, in which case a significant number of samples is produced (in parallel) by \Ac{sampler}, but never used by \Ac{EAA}. 
Although such circumstances are a clear symptom of an over-dimensioning of the hardware infrastructure, they do not pose a usability problem for the tool, since in this case the overall completion time is in the range of a few seconds or minutes.

\begin{figure}
	\footnotesize
	\addtolength{\abovecaptionskip}{-3pt}
	\renewcommand{\tabularxcolumn}[1]{m{#1}}
	%
	\newcolumntype{Y}{>{\centering\arraybackslash}X}
	\renewcommand{\tabcolsep}{0pt}
	\newcommand{\LeftYLabel}{\rotatebox[origin=c]{90}{\scriptsize time (log scale)}}
	\newcommand{\RightYLabel}{\rotatebox[origin=c]{90}{\scriptsize efficiency (linear scale)}}
	\newcommand{\XLabel}{\scriptsize\ensuremath{\Precision~(\times 10^{-2})}}
	\begin{tabularx}
		{\linewidth}
		{
			m{\widthof{~1024~}} 
			c
			*{3}{Y}
			c
		}
		  $\SimNb$
		& 		  
		& \Acs{AT}
		& \Acs{FCS}
		& \Acs{ALMA}
		\\[1ex]
		  1
		& \LeftYLabel
		& \includegraphics
			[width=\linewidth]
			{parallel_performance_AT_1workers.pdf}	
		& \includegraphics
			[width=\linewidth]
			{parallel_performance_FCS_1workers.pdf}	
		& \includegraphics
			[width=\linewidth]
			{parallel_performance_ALMA_1workers.pdf}
		& \RightYLabel 
		\\
		  128
		& \LeftYLabel
		& \includegraphics
			[width=\linewidth]
			{parallel_performance_AT_128workers.pdf}	
		& \includegraphics
			[width=\linewidth]
			{parallel_performance_FCS_128workers.pdf}	
		& \includegraphics
			[width=\linewidth]
			{parallel_performance_ALMA_128workers.pdf}	
		& \RightYLabel	
		\\
		  512
		& \LeftYLabel
		& \includegraphics
			[width=\linewidth]
			{parallel_performance_AT_512workers.pdf}	
		& \includegraphics
			[width=\linewidth]
			{parallel_performance_FCS_512workers.pdf}	
		& \includegraphics
			[width=\linewidth]
			{parallel_performance_ALMA_512workers.pdf}	
		& \RightYLabel
		\\
		  1024
		& \LeftYLabel
		& \includegraphics
			[width=\linewidth]
			{parallel_performance_AT_1024workers.pdf}
		& \includegraphics
			[width=\linewidth]
			{parallel_performance_FCS_1024workers.pdf}	
		& \includegraphics
			[width=\linewidth]
			{parallel_performance_ALMA_1024workers.pdf}
		& \RightYLabel
		\\
		  2048
		& \LeftYLabel
		& \includegraphics
			[width=\linewidth]
			{parallel_performance_AT_2048workers.pdf}	
		& \includegraphics
			[width=\linewidth]
			{parallel_performance_FCS_2048workers.pdf}	
		& \includegraphics
			[width=\linewidth]
			{parallel_performance_ALMA_2048workers.pdf}
		& \RightYLabel
		\\[-1ex]
		  % empty
		& % empty
		& \XLabel
		& \XLabel
		& \XLabel
		& % empty
	\end{tabularx}

	\caption{%
		Scalability analysis of our parallel tool: overall completion time (bottom curves, left Y log-scale axis) and efficiency (top curves, right Y axis) for each case study and selected values for the number of simulators $\SimNb$.		
	}
	\label{fig:expres:scalability}
\end{figure}

==> 06-experiments-results.tex <==
%!TEX root = ./root.tex
%
Here we present our experimental results.
Namely, in \cref{sec:expres:eaa} we quantify the benefit of using \Ac{EAA} in terms of reduction in the number of samples required to convergence, whilst in \cref{sec:expres:sampler} we exploit the methodology outlined in \cref{sec:expres:setting} to conduct a performance scalability analysis of our parallel tool.


\SectionInput
	[sec:expres:eaa]
	{Reduction of the number of required samples due to \Acs{EAA}}
	{06-experiments-results-ensemble.tex}

\SectionInput
	[sec:expres:sampler]
	{Increase of the sample production rate due to the \Acl{sampler}}
	{06-experiments-results-sampler.tex}	

\SectionInput
	[sec:expres:scalability]
	{Overall performance scalability analysis}
	{06-experiments-results-scalability.tex}	

==> 06-experiments-setting.tex <==
%!TEX root = ../../root.tex
%
Here we describe how we conducted a thorough and statistically sound analysis of the performance and scalability of our parallel tool.

For each case study we computed $\PrecConf$-approximations of the \Acp{KPI} of interest for 9 different values for $\Precision$ (ranging from \Pretty{1e-3} to \Pretty{1e-1}), 3 values of $\ConfMargin$ (\Pretty{1e-2}, \Pretty{5e-2}, \Pretty{1e-1}), and 7 values for $\SimNb$ (1, 64, 128, 256, 512, 1024, 2048). 
Each experiment has been repeated 10 times, using 10 sequences of samples, each one produced by a different sequence of \Ac{iid} scenarios.

Conducting such an analysis using our production tool of \cref{sec:expres:implementation} would be a \emph{practically unviable} option, as it would require dozens of years (see \cref{fig:expres:scalability}) and incur in huge costs for the full allocation of a large-enough private \Ac{HPC} infrastructure. 
Indeed, for a proper analysis to be carried out, the production tool would need to be run 10 times for each case study and for each value of $\Precision$, $\ConfMargin$ and $\SimNb$ (including $\SimNb = 1$).
Also, each execution of the tool would require the full availability of $\SimNb+4$ computational nodes (CPU cores), including $\SimNb + 4 = 2048 + 4 = 2052$.

This obstruction is becoming common when analyzing performance and scalability of modern software explicitly designed to perform intensive computations on large \Ac{HPC} infrastructures, and is being handled in the literature from the methodological point of view.
%
Along these lines, and by following recent approaches such as, \eg \cite{esposito-etal:2023:tsmc}, we operated in an \emph{indirect} way as follows.

First, we avoided the use of an expensive private \Ac{HPC} infrastructure, by exploiting a \emph{shared} \Ac{HPC} cluster at Sapienza University, which is managed by a centralized scheduler which orchestrates the launch of the computational jobs submitted concurrently by the various research teams.
%
Although this was a mandatory choice, it created some issues, as jobs requesting too many computational nodes to be allocated would have received a very low priority and could have remained in the waiting queue forever.

Hence, as in \cite{esposito-etal:2023:tsmc}, we \emph{disassembled} our tool into its single components, instrumented each component with proper timers within the code, and ran each of them \emph{asynchronously}. 
More precisely:

\begin{enumerate}
	\item We generated 10 random seeds for each case study and computed 10 sequences of scenarios long enough to allow all \Acp{SA} to terminate for all values of $\Precision$ and $\ConfMargin$. We saved these sequences of scenarios into a centralized database, together with their ids and generation times (which are all on the order of a few microseconds).
	
	\item We submitted to the \Ac{HPC} scheduler the simulation jobs for all scenarios independently, and measured the time taken by each of them to simulate the selected scenario and to compute the corresponding value of the system \Ac{KPI} (we ignored the simulator set-up time, which would not have had to be paid for each sample if we had instead used the production tool).
	For each scenario, the simulation time and the \Ac{KPI} value were also saved in the centralized database. 
	Note that, as expected, simulation is by far the slowest step in the whole workload, with average times being orders of magnitude higher than those of the others, namely:
		\DataGet{case studies/at/sim time/avg}, 
		\DataGet{case studies/fcs/sim time/avg},
		\DataGet{case studies/alma/sim time/avg} 
	for \Ac{AT}, \Ac{FCS} and \Ac{ALMA}, respectively.


	\item For each case study, the average half turnaround network time for each message type from \Ac{HPC-EAA} to a simulator and vice versa was measured independently, by running the real (\Ac{MPI}-based) application over \DataGet{exps/time/network/scenarios/nb} scenarios. Thanks to a low-latency high-throughput local network, these times are all on the order of a hundred of microseconds (\ie around $\Pretty[s]{1e-4}$), hence several orders of magnitude lower than simulation times.
\end{enumerate}	

We asked the \Ac{HPC} scheduler to run all the computations on nodes of identical machines, each one equipped with 2 AMD EPYC 7301 CPUs with 32 cores and 256 GB RAM, and hyper-threading disabled. 
This ensured that the measured time durations can be seamlessly combined together.

With the above data, we were able to virtually exercise our tool on 10 random experiments for each case study, assessing convergence of the \Acp{SA} and overall performance on each setting ($\Precision$, $\ConfMargin$, and $\SimNb$).
%
Indeed, the availability of the generation and simulation times of each scenario as well as of the average half turnaround time of network messages of each type allowed us to perform a reliable estimation of the execution time that our production tool would have shown, under each setting, if run over fully reserved portions of the \Ac{HPC} infrastructure at hand. 
%
Namely, for each experiment, the \Acp{SA} and \Ac{sampler} modules were run normally (as a multi-threaded process on a single node), although properly instrumented, while the set of simulators were replaced by the database containing the pre-computed samples.
A discrete event-based emulator module running on the same node (see \cite{esposito-etal:2023:tsmc}) orchestrated the execution of the whole experiment in a faster-than-real-time way, by mimicking the advancement of time via a global counter accumulating the time durations of all steps of \cref{algo:eaa,algo:sampler} (\ie scenario generation, blocking dequeue operations from the queue of available simulators, network communication to and from the simulators, blocking look-up operations and insertion/deletion of entries to/from the \AlgoVar{samples} map and advancement of all \Acp{SA}). 
The time durations of the steps performed normally were measured via the timers instrumenting the code, while those of the emulated steps were taken from the database.

We note that, although we did our best to take into account, in our estimation, also the steps which are several orders of magnitude faster than the dominating tasks (system model simulations), it is known that disassembling and instrumenting the production code can introduce unnoticed small divergences between the estimated time and the time that our tool would have shown if run normally. 
%
However, such potential small divergences would actually be \emph{unmeasurable and not repeatable} in practice. This is due to how modern large \Ac{HPC} infrastructures (even those fully reserved for a single job) are managed by complex orchestrating and probing services, and by software virtualization and containerization layers, which may introduce a significant amount of noise.

In other words, the estimations below, as all estimations of the completion time of complex massively parallel and computationally intensive software designed for large \Ac{HPC} infrastructures, actually estimate what would happen if the software would run on \emph{bare metal}.


==> 06-experiments.tex <==
%!TEX root = ./root.tex
%
In this section we present our three industrial case-study models taken from the literature, outline the implementation of our \Ac{HPC} software, and use our tool to perform model-based \Ac{SMC} verification tasks of our three models.

Our results highlight how the conjoint effects of using an ensemble of $\PrecConf$-approximation algorithms and a massively parallel architecture to perform (the expensive) scenario simulations required to provide \EAA with \Ac{iid} samples allow us to complete our verification tasks within a reasonable time frame, whereas a na{\"i}ve implementation would have been taken an \emph{inconceivably} long time.

\SectionInput
	[sec:expres:case-studies]
	{Case studies}
	{06-experiments-case-studies.tex}

\SectionInput
	[sec:expres:implementation]
	{Implementation}
	{06-experiments-implementation.tex}

\SectionInput
	[sec:expres:setting]
	{Experimental setting}
	{06-experiments-setting.tex}

\SectionInput
	{Results}
	{06-experiments-results.tex}







==> 07-conclusion.tex <==
%!TEX root = ./root.tex
\AcronymReset{CPS}
\AcronymReset{EAA}
\AcronymReset{HPC}
\AcronymReset{SA}
\AcronymReset{SMC}
In this article, we focused on the simulation-based verification of complex systems with \Ac{SMC}, by highlighting how \Acp{SA} form a class of approximation algorithms well-suited for parallelization. 
Not only their design make the parallelization of the generation of the system simulations (samples) possible, but it also allows them to be combined without any interference or complication. 

We proposed \Ac{EAA}, a composite algorithm combining the respective strengths of multiple \Acp{SA}. 
We successfully implemented and tested \Ac{EAA} exploiting two (quasi) optimal algorithms: \EBGStop and \ApproxAlgo, together with a massively parallel architecture deployable over large \Ac{HPC} infrastructures.

We exercised our tool on three industry-scale case studies, verifying specifications of non-trivial properties, and showed that parallelization can indeed make \Ac{SMC} a viable approach for the verification of complex systems, even when the number of required simulations can appear prohibitive from a sequential perspective.
%
We exposed an in-depth experimental analysis of our tool, detailing the benefits of combining multiple \Acp{SA}, quantifying the effective reductions in sample sizes and execution times, and discussing the efficiency of the parallelization and the impact of the number of parallel simulators.
%
All in all, our work makes it clear that parallelization should be considered as systematically as possible to increase and widen the applicability of \Ac{SMC}.

\medskip

A direct extension of \Ac{EAA} would obviously be one which integrates other \Acp{SA}, potentially making it even more versatile and applicable to a larger class of \Acp{KPI}.

To go further, our tool could be expanded to allow for the verification of formula-based properties, expressed for instance in linear temporal logic. In its simplest form, this would be effortless, since the probability than a chosen property holds for a random possible execution of a system can be seen as a \Ac{KPI} of that system. 
A more ambitious plan would be to explore whether a strategy such as the one behind the elaboration of \Ac{EAA} could help for the verification of hyper-properties \cite{arora2022statistical,dobe2023lightweight}.

Repeating the analysis of the impact of parallelization on the effectiveness and applicability of \Ac{SMC} with a composite algorithm combining multiple optimization algorithms rather than simple estimation algorithms would be interesting. Identifying a class of optimization algorithms for \Ac{SMC} which share some of the key properties of stopping algorithms that make their parallelization relatively straightforward would be a first step.

Our tool could then also be enhanced even further by improving the sampling process itself, similarly to what has been done in \cite{parmentier2023optimized}, especially when taking into account geometric sampling. 



==> 08-acknowledgements.tex <==
%!TEX root = ./root.tex
This work was partially supported by: 
%
INdAM ``GNCS Project 2023''; 
%
Sapienza University projects 
  RG12117A8\-B393BDC% 2021-2024 - VPH grande (T. Mancini)
, RM120172B9F35634% 2020-2023 - Virtual doctor
, RG123188B482D2D9% 2023-2026 - Virtual doctor (PI: Ferracuti)
;
%
Lazio POR FESR projects 
  E84G20000150006% SDFS
, F83G170\-00830007% SCAPR
;
%
Project funded under the National Recovery and Resilience Plan (NRRP), Mission 4 Component 2 Investment 1.5 - Call for tender No.\ 3277 of 30 December 2021 of the Italian Ministry of University and Research funded by the European Union – NextGenerationEU, award number: project ECS 0000024 Rome Technopole, Concession Decree No. 1051 of 23 June 2022 adopted by the Italian Ministry of University and Research, CUP B83C22002820006, Rome Technopole.
%%% OR, IN SHORT:
%%% NRRP NRRP ECS 0000024, Mission 4, Comp.\ 2, Inv.\ 1.5, NextGenEU, MUR CUP B83C22002820006, Rome Technopole.

M.\ Parmentier is funded by a FNRS PhD Grant and by the UCLouvain. A.\ Legay is funded by a FNRS PDR - T013721.

